MoPe: Model Perturbation-based Privacy Attacks on Language Models

Recent work has shown that Large Language Models (LLMs) can unintentionally leak sensitive information present in their training data. In this paper, we present Model Perturbations (MoPe), a new method to identify with high confidence if a given text is in the training data of a pre-trained language model, given white-box access to the models parameters. MoPe adds noise to the model in parameter space and measures the drop in log-likelihood at a given point $x$, a statistic we show approximates the trace of the Hessian matrix with respect to model parameters. Across language models ranging from $70$M to $12$B parameters, we show that MoPe is more effective than existing loss-based attacks and recently proposed perturbation-based methods. We also examine the role of training point order and model size in attack success, and empirically demonstrate that MoPe accurately approximate the trace of the Hessian in practice. Our results show that the loss of a point alone is insufficient to determine extractability -- there are training points we can recover using our method that have average loss. This casts some doubt on prior works that use the loss of a point as evidence of memorization or unlearning.

==> extract.tex <==
\section{Training Data Extraction}
\label{sec:extract}
With LLMs being generative models, membership inference attacks can be more dangerous as they may potentially be used for explicit training data extraction. In particular, we borrow the extraction attack methodology from \cite{yu2023bag} to test the performance of MoPe for such a task. Let $x_1,\dots,x_M$ be prefixes (prompts) to attack with ground truth suffixes $y_1,\dots,y_M$. (i) For $i = 1 \dots M$ generate $N$ synthetic samples from an LLM $\theta$: $s_{i_1},\dots,s_{i_N} \stackrel{iid}{\sim} p_{\theta | x_i}$. (ii) Using the membership inference attack $\mathcal{A}$ rank the generated samples according to likelihood of training set membership. (iii) Predict the most likely suffix for each prefix or the top $k \ll N$ likely suffixes over all prefixes as training samples. Some metrics of interest include exact match accuracy $\mathrm{EMA}(s)=\sum_{i=1}^M I(y_i=s_{i_{lowest}})$ and token level accuracy $\mathrm{TLA}(s)=\sum_{i=1}^M\sum_{j=1}^{|s_i|}I(y_i^{(j)}=s_{i_{lowest}}^{(j)})$ where the superscript denotes token-level index. These are related to precision and (inverse) Hamming distance in \cite{yu2023bag} respectively. Additional metrics of interest include any match accuracy (if any predicted suffix for a prefix is an exact match), recall at 100 errors (the metric used in the Google Extraction Challenge), and AUC over the entire set of generated suffixes.

Using the Google Extraction Challenge dataset, we test LOSS and MoPe for this attack pipeline on 1000 samples and across different sizes of GPT Neo, the model for which this challenge was designed for. We use the autotuned sampling hyperparameters given by \cite{yu2023bag}\footnote{Top-24, nucleus 0.8, typical 0.9, temperature 0.58, repetition penalty 1.04.}.

\begin{table}[h]
\small
\begin{tabular}{|l|ll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{125M} & \multicolumn{2}{c|}{1.3B} & \multicolumn{2}{c|}{2.7B} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{LOSS} & MoPe & \multicolumn{1}{l|}{LOSS} & MoPe & \multicolumn{1}{l|}{LOSS} & MoPe \\ \hline
Exact Match Acc & \multicolumn{1}{l|}{0.202} & 0.147 & \multicolumn{1}{l|}{0.505} & 0.396 & \multicolumn{1}{l|}{0.580} &  \\ \hline
Token Level Acc & \multicolumn{1}{l|}{0.389} & 0.338 & \multicolumn{1}{l|}{0.684} & 0.604 & \multicolumn{1}{l|}{0.753} &  \\ \hline
Any Exact Acc & \multicolumn{1}{l|}{0.225} & 0.221 & \multicolumn{1}{l|}{0.551} & 0.546 & \multicolumn{1}{l|}{0.629} &  \\ \hline
Recall at 100 Errors & \multicolumn{1}{l|}{0.858} & 0.103 & \multicolumn{1}{l|}{0.955} & 0.282 & \multicolumn{1}{l|}{0.952} &  \\ \hline
AUC & \multicolumn{1}{l|}{0.935} & 0.414 & \multicolumn{1}{l|}{0.876} & 0.334 & \multicolumn{1}{l|}{0.880} &  \\ \hline
\end{tabular}
\end{table}

EXAMPLES

DISCUSSION of RESULTS

% \begin{itemize}
%     \item Describe the basic pipeline: for each prefix, we generate 100 suffixes, and rank the top 5 using MoPe and using loss. For each of these 5, we check if any are in the training set. We report the accuracy e.g. number of suffixes where at least one of the five generations was correct, out of the 1000.
%     \item We're worried GPTNeoX1.3B will not have good results because MoPe doesn't work super well; should we try a smaller model from the same family? Need to verify that training data is the same before we try this.... 
%     \item For both methods use the sampling parameters from Bag of Training paper
%     \item Can we show some examples of extracted strings, that we can extract with MoPe but not with LOSS?

\end{itemize}

==> grad.tex <==
\section{First-Order Gradient-Based Thresholding}
\label{sec:grad}

Given the large computational footprint and approximation nature of MoPe for calculating the trace of the Hessian, we also explore a novel attack based on thresholding the norm of the gradient. This requires only one inference per point, and involves the same memory as would be required for training the model. The intuition behind the success of this attack is that after training, the model loss on training points are more likely to be at local minima, which entails a small gradient norm. Unfortunately, this attack may also pick up local maxima as training points, which is why a combination of LOSS, GRAD, and MoPe may paint the fullest picture of the model's loss landscape. Given the large memory footprint of this method, we only run up to the 2.8B model, and we evaluate the method on L1, L2, and L$\infty$ norms, and compare across the gradient with respect to the input text (in a vein similar to DetectGPT) and with respect to the model parameters (which supports the motivating visual intuition). The results in Table \ref{tab:grad} indicate the large success of this attack, but also its variability. L$\infty$ norm appears to be the best, reflecting the idea that even if a single dimension has high derivative, then it is not a true local minima. There is an unexplained dip in performance with the 2.8B Pythia model and the gradient with respect to the input, and the gradient with respect to the model parameters shows basically random performance for the 70m and 160m models, but interestingly does well for larger models.



\begin{table}[h]
\centering
\caption{GRAD Attack}
\label{tab:grad}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{3}{c|}{AUC for $||\nabla_x\ell(x, \theta)||_p$} & \multicolumn{3}{c|}{AUC for $||\nabla_\theta \ell(x, \theta)||_p$} & \multicolumn{2}{c|}{Perturbed} & \multicolumn{1}{c|}{Loss} \\ \cline{2-10} 
\multicolumn{1}{|c|}{} & $p = 1$ & $p = 2$ & $p = \infty$ & $p = 1$ & $p = 2$ & $p = \infty$ & $\mope$ & DetectGPT  & $\loss$ \\ \hline
70m & $0.4998$ & $0.5305$ & $0.5781$ & $0.4706$ & $0.4937$ & $0.5000$ & $\bm{0.6069}$ & & $0.5075$ \\ \hline
160m & $0.5574$ & $0.5592$ & $0.5867$ & $0.4653$ & $0.5176$ & $0.5090$ & $\bm{0.6478}$ & & $0.5118$  \\ \hline
410m & $0.5361$ & $0.5369$ & $0.5394$ & $0.4107$ & $0.5555$ & $\bm{0.6517}$ & $0.5958$ & & $0.5135$  \\ \hline
1b & $0.6323$ & $0.6316$ & $\bm{0.6466}$ & $0.2826$ & $0.6323$ & $0.5795$ & $0.5924$ & & $0.5161$ \\ \hline
1.4b & $\bm{0.6119}$ & $0.6106$ & $0.6094$ & $0.3496$ & $0.5891$ & $0.5924$ & $0.5656$ & & $0.5168$ \\ \hline
2.8b & $0.4883$ & $0.4901$ & $0.4918$ & $0.1789$ & $0.5853$ & $\bm{0.6300}$ & $0.5320$ & & $0.5039$ \\ \hline
6.9b & $0.6350$ & $0.6329$ & $0.6120$ & $0.2222$ & $0.5803$ & $\bm{0.6526}$ & $0.5217$ & & $0.5227$ \\ \hline
12b & & & & & & & $0.5164$ & & $0.5252$ \\ \hline
\end{tabular}
\end{table}







